Explicit Formula for Partial Information Decomposition

Mutual information between two random variables is a well-studied notion, whose understanding is fairly complete. Mutual information between one random variable and a pair of other random variables, however, is a far more involved notion. Specifically, Shannon's mutual information does not capture fine-grained interactions between those three variables, resulting in limited insights in complex systems. To capture these fine-grained interactions, in 2010 Williams and Beer proposed to decompose this mutual information to information atoms, called unique, redundant, and synergistic, and proposed several operational axioms that these atoms must satisfy. In spite of numerous efforts, a general formula which satisfies these axioms has yet to be found. Inspired by Judea Pearl's do-calculus, we resolve this open problem by introducing the do-operation, an operation over the variable system which sets a certain marginal to a desired value, which is distinct from any existing approaches. Using this operation, we provide the first explicit formula for calculating the information atoms so that Williams and Beer's axioms are satisfied, as well as additional properties from subsequent studies in the field.

==> Axioms_2.tex <==
\section{Framework and Desired Properties}

%\red{[Before mentioning the axiomatic approach to PID, mention the axiomatic approach to mutual information~\cite{csiszar2008axiomatic}: (A) Characterization of functions of probability distributions suitable as information measures. (B) Characterization of set functions on the subsets of {1,…,N} representable by joint entropies of components of an N-dimensional random vector. (C) Axiomatic characterization of MaxEnt and related inference rules. ]}

The establishment of PID is based on an axiomatic approach, which involves first proposing a set of axioms that the method should satisfy and then giving a definition and proving the satisfaction. This approach has precedents in the field of information theory, such as the strict axiomatic approach for mutual information \cite{csiszar2008axiomatic}. In this section, we will sort out the axioms and related properties of PID to provide support for the methods and proofs proposed in the next section.

PID is a framework for decomposing the mutual information between a set of source variables and a target variable into non-overlapping directional information atoms \cite{williams2010nonnegative}. In the three-variable scenario $\{X,Y,Z\}$ shown in Figure \ref{fig:PID}, it can be written as:
\begin{align}
I(X,Y;Z)= &Red(X,Y \to Z) +Syn(X,Y \to Z)\nonumber \\&+Un(X\to Z\vert Y)+ Un(Y\to Z\vert X)
\end{align}

As a group of more fine-grained information measures ($f:\mathcal{D} \to \mathbb{R}$), information atoms enable the further division of measures such as mutual information and conditional entropy: 
Redundant information $Red(X,Y\to Z)$ ($Red_{XY-Z}$) represents the information shared by the source variable $X,Y$ and provided to the target variable $Z$. Unique information $Un(X \to Z|Y)$($Un_{X-Z}$) refers to the information individually contributed to $Z$ by the source variables $X$ (the same goes for $Un(Y \to Z|X)$). Therefore, for every source variable $X$ or $Y$, its unique and redundant information constitutes all the information it provides to the target variable, which is the mutual information, such that:
\begin{align}
Red(X,Y \to Z) + &Un(X\to Z\vert Y) = I(X;Z)\\
Red(Y,X \to Z) + &Un(Y\to Z\vert X) = I(Y;Z)
\end{align}
\red{[Appears in many places, provide citation to e.g., \cite[Eq.~(1)-(3)]{bertschinger2014quantifying}, \cite[Eq.~(1)]{rauh2023continuity}]} \red{These formulas have been clearly given in the first article, and subsequent articles just repeat. Do we need to quote them?}

In addition to the above two kinds of information atoms, the joint mutual information $I(X,Y;Z)$ also contains synergistic information $Syn(X,Y\to Z)$ ($Syn_{XY-Z}$), which is the information that can only be known about $Z$ through the joint observation of $X$ and $Y$ but cannot be provided by a single source variable. The following is a formal expression of those information atoms \cite{williams2010nonnegative}: 
\begin{axiom}[Information Atoms' relationship] 
\label{def: Information Atoms' relationship}
In a system with variables $X,Y,Z$, we have
\begin{align}
I(X,Y;Z)= &Red(X,Y \to Z) +Syn(X,Y \to Z) \nonumber \\&+Un(X\to Z\vert Y)+ Un(Y\to Z\vert X)\\
\label{equ:Information Atoms' relationship_2}
I(X;Z) = &Red(X,Y \to Z) + Un(X\to Z\vert Y)\\
\label{equ:Information Atoms' relationship_3}
I(Y;Z) = &Red(X,Y \to Z) + Un(Y\to Z\vert X)\\
Syn(X,Y \to Z) + &Un(X\to Z\vert Y) + H(Z|X,Y)= H(Z|Y)\\
Syn(X,Y \to Z) + &Un(Y\to Z\vert X) + H(Z|X,Y)= H(Z|X)
\end{align}
\end{axiom}  

%\label{def: Information Atoms' relationship}

%\begin{axiom} [Information Atoms' relationship] In a system with variables $X,Y,Z$, we have \begin{align}
%Red(X,Y \to Z) +&Un(X\to Z\vert Y)+ Un(Y\to Z\vert X)\nonumber \\
%+Syn&(X,Y \to Z)=I(X,Y;Z)\\
%        Red(X,Y \to Z) + &Un(X\to Z\vert Y) = I(X;Z)\\
%        Red(X,Y \to Z) + &Un(Y\to Z\vert X) = I(Y;Z)\\
%        Syn(X,Y \to Z) + &Un(X\to Z\vert Y) + H(Z|X,Y)= H(Z|Y)\\
%        Syn(X,Y \to Z) + &Un(Y\to Z\vert X) + H(Z|X,Y)= H(Z|X)
%\end{align}

%The term~$Un(X\to Z\vert Y)$ reflects the information that~$X$ implies about~$Z$ given that~$Y$ is known, and hence it is a strictly directional concept. 
%By our intuitive understanding of Fig.~\ref{fig:PID},  $Red_{XY-Z}$ is not directional in the sense that both~$X$ and~$Y$ contribute this part of the information to~$Z$, and the commutativity $Red_{XY-Z}=Red_{YX-Z}$ must hold. Therefore, to get both this form of commutativity and the compatibility with Shannon's formula we must have that
%\begin{align}\label{equation:CommutativeRed}
    %I(X;Z)-Un(X\to Z\vert Y)=I(Y;Z)-Un(Y\to Z|X).
%\end{align}

%\red{need more explanation. (physical meaning)} Similarly, by our intuitive understanding of Fig. \ref{fig:PID}, since $I(X,Y;Z)=H(Z)-H(Z|X,Y)$, $Syn_{X,Y\to Z}$ also needs to satisfy the Axiom: 

\begin{figure}[htbp]
\centering
\fbox{\includegraphics[width=.9\linewidth]{image/PID_Venn.png}}
\caption{Venn diagram of PID.}
\label{fig:PID}
\end{figure}

The above formulas provide a set of constraints on the relationships between all information atoms but do not specify the value of each. Therefore, we need to formulate a numerical definition of one of those information atoms so that the values of the others can be obtained through those relationships. In Williams and Beer's paper, they chose redundant information as the starting point and gave three axioms that redundant information should satisfy \cite{williams2010nonnegative,lizier2013towards}.

The first is the commutativity of the source variables, that means the order of the source variables does not affect the value of redundant information. The second is monotonicity of redundancy, that the redundant information is non-increasing when adding source variable, since the newly added variable cannot increase the redundancy between the original variables but further reduce it. The third one is called self-redundancy, which define the redundant information from one source variable to target variable as the mutual information between them. That gives a special definition of redundant information in two variables case, making the information decomposition framework fully compatible with existing measures such as mutual information. 

In this paper, we mainly focus on the three-variable case, and the above axioms can be formally written as follows, where monotonicity and self-redundancy can be merged into one:

%However, $Syn_{XY-Z}$ should inherently not depend on the order of~$X,Y$; this is a quantity which reflects the information which $X$ and$Y$ jointly imply about~$Z$. However, the \red{equation} shown above can potentially depend on the order between~$X$ and~$Y$. Therefore, we define
%, 
%and similarly~$Syn_Z(X;Y)=...$. To get both the required intuitive commutativity and the compatibility with Shannon's formula, we have the following axiom.
% \begin{align*}
% Un(X \to Z | Y) + Red((X,Y)\to Z) &= I(X;Z),  \\
% Un(Y \to Z | X) + Red((Y,X)\to Z) &= I(Y;Z), \\
% Un(X \to Z | Y) + Syn(X,Y\to Z) &= H(Z|Y) - H(Z|X,Y),\mbox{ and}\\
% Un(Y \to Z | X) + Syn(Y,X\to Z) &= H(Z|X) - H(Z|X,Y).
% \end{align*}

\begin{axiom} [Commutativity]
\label{Axiom: Commutativity}
Redundant information is invariant under any permutation of sources. For the system with source $X,Y$ and target $Z$, it can be write as:
\begin{align}
Red(X,Y\to Z) = Red(Y,X\to Z) 
%Syn(X,Y\to Z) = Syn(Y,X\to Z) 
\end{align}
\end{axiom}    

%\begin{axiom} [Monotonicity of redundant information]
%\label{Axiom:Monotonicity}
%The redundant information from source variables $\{X\}$ to the target $Y$ should exhibit a monotonically decreasing behavior with the inclusion of additional inputs. \red{[Write in a 3-variable form, and unite Axioms 2 and 3. Can mention that they should be split for~$>3$ variables in a footnote. Perhaps add a paragraph explaining why the united axiom is called monotonicity.]}
%\begin{align} 
%Red(X_{1},\cdots,X_{n} \to Y) \le  Red(X_{1}, \cdots ,X_{n}\setminus X_{i} \to Y) \nonumber \\ \forall i \in \{1, \cdots, n\}
%\end{align}
%\end{axiom}

%\begin{axiom} [Self-redundancy]
%\label{axiom:Self-redundancy}
%When there are only two variables, the redundant information is equivalent to the mutual information
%\begin{align} 
%Red(X_{1} \to X_{2}) = I(X_{1};X_{2})
%\end{align}
%\end{axiom}

\begin{axiom} [Monotonicity and Self-redundancy]
\label{axiom: Monotonicity and Self-redundancy}
For the system with source $X,Y$ and target $Z$, the unique information is less than the mutual information between each source and target.
\begin{align} 
Red(X,Y \to Z) \le \min_{S\in\{X,Y\}}I(S;Z)
\end{align}
\end{axiom}

%Since information decomposition is a further decomposition of information measures such as mutual information and conditional entropy, it should be naturally compatible with those measures. Although not explicitly stated, the Figure \ref{fig:PID} and Axiom \ref {axiom:Self-redundancy} implies  Therefore the following axiom (\red{we expanded}) states that the information atoms should adhere to known conventions regarding mutual information. 



%, as depicted by the famous Venn diagram \ref{fig:Venn diagram for two variables}.

%\begin{figure}[htbp]
%\centering
%\fbox{\includegraphics[width=.8\linewidth]{image/Info.png}}
%\caption{Venn diagram for two variables.}
%\label{fig:Venn diagram for two variables}
%\end{figure}

In addition, considering that redundant information serves as a non-negative alternative measure of interactive information and as the title of the original paper \cite{williams2010nonnegative}, PID should be a set of non-negative measures, just like other information measures such as mutual information and information entropy. Therefore we can write this axiom explicitly:

\begin{axiom} [Nonnegativity]
\label{Axiom: Nonnegativity}
The values of redundant information atoms are non-negative real numbers.
\begin{align} 
\label{equ: Nonnegativity_1}
Red(X,Y \to Z) \ge 0
\end{align}
\end{axiom}

\red{[Mention continuity (in the probability distribution) as a requirement?]}

\red{[I'am not sure. According to \cite{rauh2023continuity}, most of the existing methods satisfy it. I have done experiments and our method satisfies it, but I may need some time to prove it.]}


In addition, considering PID as an information measure, it should also satisfy additivity and continuity \cite{bertschinger2014quantifying} \cite{rauh2023continuity}. 

Additivity means when independent variables are considered jointly, the joint information measure should be the sum of partial information measures. For example, the joint entropy of two independent variables is equal to the sum of their respective entropies. So far, \cite{bertschinger2014quantifying} is the only definition of an information atom that satisfies this property\cite{rauh2023continuity}:

\begin{property} [Additivity] 
\label{property: Additivity}
For two independent probability distributions, $\mathcal{D}_{(X_1,X_2,X_3)}$ and $\mathcal{D}_{(A_1,A_2,A_3)}$, we have:
\begin{align}
Red(X_i,X_j\to X_k) + Red(A_l,A_m\to A_n)\nonumber \\
= Red((X_i,A_l),(X_j,A_m)\to (X_k,A_n)) \\
Syn(X_i,X_j\to X_k) + Syn(A_l,A_m\to A_n)\nonumber \\
= Syn((X_i,A_l),(X_j,A_m)\to (X_k,A_n))  \\
Un(X_i \to X_j | X_k) + Un(A_l\to A_m | A_n)\nonumber \\
= Un((X_i,A_l) \to (X_j,A_m) | (X_k,A_n)) \\
i,j,k,l,m,n \in \{1,2,3\} \nonumber 
\end{align}
\end{property}


Continuity refers to the behavior of the information measure when the probability distribution changes slightly. Specifically, it means that small changes in the probability distribution should lead to small changes in the value of the information measure. Continuity ensures that the measure behaves predictably and is a key property in information theory, particularly for measures like entropy and mutual information.

\begin{property} [Continuity] 
\label{property: Continuity}
The redundant, unique and synergistic information shouldn't produce drastically different values for minor variations in the probabilities.
\end{property}

Another well-known property is Independent Identity Property, which was proposed by Ince\cite{ince2017measuring}. This property is based on an intuitive case called Copy Gate: When two independent variables are decomposed together into their joint variable, the redundant information should be 0:

\begin{property}[Independent Identity]
\label{property: Independent Identity}
For any redundant information measure $Red(X_1,X_2\to Y)$, if $I(X_1,X_2)=0$ and $Y=(X_1,X_2)$, then
\begin{align}
    Red(X_1,X_2\to Y) = 0
\end{align}
\end{property}

In addition to the axioms and properties listed above, there are some common properties that are not listed but can be derived from the above constraints. For example, the non-negativity of unique information can be obtained from Axiom \ref{def: Information Atoms' relationship} and Axiom \ref{Axiom: Nonnegativity}; the commutativity of synergistic information obtained from Axiom \ref{def: Information Atoms' relationship} and Axiom \ref{Axiom: Commutativity}; the consistency \cite{bertschinger2014quantifying} can be obtained from the difference between equation (\ref{equ:Information Atoms' relationship_2}) and (\ref{equ:Information Atoms' relationship_3}), etc.


\red{[TO ADD: More detailed technical references to previous works about PID, and their flaws~\cite{bertschinger2014quantifying,banerjee2018computing,venkatesh2022partial,niu2019measure,james2018unique}.}

[This would take up a lot of space and is not exhaustive. I think it is better to intersperse the comparison with the introduction of the axioms. Detailed comparisons can be left to later journal editions]


%1. Blackwell Case
%2. Copy Gate

%We argue that any meaningful measure for multi-variate mutual information must satisfy the following axioms from SID:

%\begin{axiom} [Symmetry of redundant and synergistic information]
%\label{Axiom:Symmetry of variables}
%$Red(X_1,\cdots,X_n)$ is invariant to the permutation of $X_i$, $\forall i \in \{1,\cdots,n\}$. Combining with Axiom \ref{Axiom: Compatible with Shannon's formula}, we can also derive the symmetry of synergistic and unique information.
%\end{axiom}



